Measurement of the shape of the $B_s^0\rightarrow D_s^{*-}\mu^{+}\nu_{\mu}$ differential decay rate

The shape of the $B_s^0\rightarrow D_s^{*-}\mu^+\nu_{\mu}$ differential decay rate is obtained as a function of the hadron recoil using proton-proton collision data at a centre-of-mass energy of 13 TeV, corresponding to an integrated luminosity of 1.7 fb$^{-1}$ collected by the LHCb detector. The $B_s^0\rightarrow D_s^{*-}\mu^+\nu_{\mu}$ decay is reconstructed through the decays $D_s^{*-}\rightarrow D_s^{-}\gamma$ and $D_s^{-}\rightarrow K^-K^+\pi^-$. The differential decay rate is fitted with the Caprini-Lellouch-Neubert (CLN) and Boyd-Grinstein-Lebed (BGL) parametrisations of the form factors, and the relevant quantities for both are extracted.

==> LHCb_Authorship_17-Dec-2019_arXiv.tex <==
LHCb collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
S. Baker,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista Leite,
A. Baranov,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
V. Batozskaya,
B. Batsukh,
A. Battig,
A. Bay,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
S. Bifani,
P. Billoir,
F.C.R. Bishop,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
E. Buchanan,
A. B{\"u}chler-Germann,
A. Buonaura,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calero Diaz,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
A. Camboni,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
K. Carvalho Akiba,
A. Casais Vidal,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
R. Cenci,
J. Cerasoli,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
V. Chekalina,
C. Chen,
S. Chen,
A. Chernov,
S.-G. Chitic,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
N. Cooke,
G. Coombs,
S. Coquereau,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
A. Crocombe,
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
J.A. de Vries,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
V. Dobishuk,
A.M. Donohoe,
F. Dordei,
M. Dorigo,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
K. Dreimanis,
M.W. Dudek,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
R. Ekelhof,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
A. Falabella,
J. Fan,
Y. Fan,
B. Fang,
N. Farley,
S. Farry,
D. Fazzini,
P. Fedin,
M. F{\'e}o,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
W. Funk,
E. Gabriel,
T. Gaintseva,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
D. Gascon,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
A. Giovent{\`u},
O.G. Girard,
P. Gironella Gironell,
L. Giubega,
C. Giugliano,
K. Gizdov,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
M. Goncerz,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
P. A. G{\"u}nther,
X. Guo,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
S.C. Haines,
P.M. Hamilton,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
R. Hart,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
P.H. Hopchev,
J. Hu,
J. Hu,
W. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
T. Humair,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
J.M. Kariuki,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
L. Li,
P. Li,
P.-R. Li,
X. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
P. Ling,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
S. Liu,
X. Liu,
D. Loh,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
Y. Lu,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
G. Meier,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M.-N. Minard,
O. Mineev,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden,
A. Mogini,
R.A. Mohammed,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mukherjee,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
I. Neri,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
D.P. O'Hanlon,
R. Oldeman,
C.J.G. Onderwater,
J. D. Osborn,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
A. Philippov,
L. Pica,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
Resmi  P.K,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
D.S. Richards,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
S. Roiser,
A. Rollings,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
C. Sanchez Gras,
C. Sanchez Mayordomo,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
S. Sellam,
A. Semennikov,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
V. Shevchenko,
E.B. Shields,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
I.T. Smith,
M. Smith,
A. Snoch,
M. Soares,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
S. Stone,
M.E. Stramaglia,
M. Straticiuc,
D. Strekalina,
S. Strokov,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
Z. Tang,
T. Tekampe,
F. Teubert,
E. Thomas,
K.A. Thomson,
M.J. Tilley,
V. Tisserand,
S. T'Jampens,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
D. Torres Machado,
D.Y. Tou,
E. Tournefier,
M. Traill,
M.T. Tran,
E. Trifonova,
C. Trippl,
A. Trisovic,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
M. van Beuzekom,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D. Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
P. Vincent,
G. Vitali,
A. Vitkovskiy,
A. Vollhardt,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
S.G. Weber,
D. Websdale,
A. Weiden,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
T. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
H. Xing,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
D. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
W.C. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhou,
Y. Zhou,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli,
D. Zuliani,
G. Zunica

==> local-symbols-def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Packages we need
\RequirePackage{xspace}

% fit outputs
\def\rhofolded        {1.142\xspace}
\def\statrhofoldedtot {0.072\xspace}
\def\statrhofolded    {0.041\xspace}
\def\systrhofolded    {0.068\xspace}

\def\rhounfolded        {1.159\xspace}
\def\statrhounfoldedtot {0.077\xspace}
\def\statrhounfolded    {0.052\xspace}
\def\systrhounfolded    {0.068\xspace}

\def\aoneunfolded        {-0.0019\xspace}
\def\stataoneunfoldedtot {0.0525\xspace}
\def\atwounfolded        {0.93\xspace}
\def\statatwounfoldedtot {0.14\xspace}
\def\stataoneunfolded    {0.034\xspace}
\def\systaoneunfolded    {0.046\xspace}
\def\statatwounfolded    {0.09\xspace}
\def\systatwounfolded    {0.10\xspace}

\def\aonefolded        {0.0320\xspace}
\def\stataonefoldedtot {0.0095\xspace}
\def\stataonefolded    {0.0055\xspace}
\def\systaonefolded    {0.0090\xspace}


% More semantic name than texttt
\newcommand{\functor}[1]{\texttt{#1}\xspace}

% Beauty decays
\newcommand{\BsToDsmunu}{\decay{\Bs}{\Dsm \mup \neum}}
\newcommand{\BsToDstaunu}{\decay{\Bs}{\Dsm \taup \neut}}
\newcommand{\BsToDssmunu}{\decay{\Bs}{\Dssm \mup \neum}}
\newcommand{\BsToDsstaunu}{\decay{\Bs}{\Dssm \taup \neut}}
\newcommand{\BsToDsslnu}{\decay{\Bs}{\Dssm (\rightarrow \Dsm\gamma) \ellp \neul}}
\newcommand{\BsToDsslnuinc}{\decay{\Bs}{\Dssm (\rightarrow \Dsm(\gamma/\piz)) \ellp \neul}}
\newcommand{\BsToDsonemunu}{\decay{\Bs}{\Dsonem \mup \neum}}
\newcommand{\BsToDsonetaunu}{\decay{\Bs}{\Dsonem \taup \neut}}
\newcommand{\BsToDsonelnu}{\decay{\Bs}{\Dsonem \ellp \neul}}
\newcommand{\BsToDszlnu}{\decay{\Bs}{\Dszm \ellp \neul}}
\newcommand{\BsToDssmuX}{\decay{\Bs}{\Dssm \mup \neum X}}
\newcommand{\BsToDsmuX}{\decay{\Bs}{\Dsm \mup X}}
\newcommand{\BsToDsPi}{\decay{\Bs}{\Dsm \pip}}
\newcommand{\BsToDsK}{\decay{\Bs}{\Dsm \Kp}}
\newcommand{\BsToDsstK}{\decay{\Bs}{\Dssm \Kp}}
\newcommand{\BdToDsPi}{\decay{\Bd}{\Ds \pim}}
\newcommand{\BsToDsRho}{\decay{\Bs}{\Dsm \rhop}}
\newcommand{\BsToDsstRho}{\decay{\Bs}{\Dssm \rhop}}
\newcommand{\BsToDsstPi}{\decay{\Bs}{\Dssm \pip}} 
\newcommand{\BToJpsiK}{\decay{\Bp}{\jpsi \Kp}}
\newcommand{\BsToDsstgPi}{\decay{\Bs}{\Dsm \g \pip}} 
\newcommand{\BsToDsstpizPi}{\decay{\Bs}{\Dsm \piz \pip}} 
\newcommand{\LbToLcPi}{\decay{\Lb}{\Lc \pim}}
\newcommand{\HbToDssHc}{\decay{H_b}{\Dssm H_c}}
\newcommand{\HcTomunu}{\decay{H_c}{\mup \neum X}}
\newcommand{\BuToDssKMuNu}{\decay{\Bm}{\Dssm \Kp \mup\neum}}
\newcommand{\BsToDssPiPiMuNu}{\decay{\Bs}{\Dssm \pip \pim \mup\neum}}
\newcommand{\BsToDssPizMuNu}{\decay{\Bs}{\Dssm \piz \mup\neum}}
\newcommand{\BdToDsttaunu}{\decay{\Bu}{\Dstarz \taup\neut}}
\newcommand{\BdToDstmunu}{\decay{\Bu}{\Dstarz \mup\neum}}

% double charm
\newcommand{\BsToDssD}{\decay{\Bs}{\Dss\D^{(*-)}_s}}
\newcommand{\BdToDssD}{\decay{\Bd}{\Dss\D^{(*-)}}} 
\newcommand{\BuToDssD}{\decay{\Bu}{\Dss\Dstarzb}} 
\newcommand{\LbToDssLc}{\decay{\Lb}{\Dssm\Lambda^{(*+)}_c}}
\newcommand{\BsToDsstHc}{\decay{\Bs}{\Dssm H_c}}
\newcommand{\BdToDsstHc}{\decay{\Bd}{\Dss H_c}}
\newcommand{\BuToDsstHc}{\decay{\Bu}{\Dss H_c}}
\newcommand{\LbToDsstHc}{\decay{\Lb}{\Dssm H_c}}
\newcommand{\BuToDsstDz}{\decay{\Bu}{\Dss\Dz}}
\newcommand{\BuToDsstDstz}{\decay{\Bu}{\Dss\Dstarzb}}
\newcommand{\LbToLcDsst}{\decay{\Lb}{\Dssm\Lcbar}}
\newcommand{\BsToDsstDsst}{\decay{\Bs}{\Dssp \Dssm}}
\newcommand{\BsToDsstDs}{\decay{\Bs}{\Dss \Dsm}}
\newcommand{\BdToDsstDm}{\decay{\Bd}{\Dss \Dm}}
\newcommand{\BdToDsstDst}{\decay{\Bd}{\Dss \Dstarm}}

% Charm decays
\newcommand{\DsToKKpi}{\decay{\Dsm}{\Km \Kp \pim}}
\newcommand{\DssToDsg}{\decay{\Dssm}{\Dsm \g}}
\newcommand{\DssToDspiz}{\decay{\Dssm}{\Dsm \piz}}
\newcommand{\LcToPKPi}{\decay{\Lc}{\proton \Km \pip}}
\newcommand{\DtomunuX}{\decay{Hc}{\mup \nu X}}
\newcommand{\DptopipiK}{\decay{\Dp}{\Km \pip \pip}}
\newcommand{\DstopipiK}{\decay{\Dsm}{\Km \pip \pim}}
\newcommand{\BtojpsiX}{\decay{B}{\jpsi(\rightarrow\mup\mun) X}}
\newcommand{\Dztokpi}{\decay{\Dz}{\Km\pip}}
\newcommand{\DspToDzpis}{\decay{\Dstarp}{\Dz(\rightarrow \Km\pip) \pi_{soft}^+}}
\newcommand{\DspToDzkkpis}{\decay{\Dstarp}{\Dz(\rightarrow \Kp\Km) \pi_{soft}^+}}
\newcommand{\Dstophipi}{\decay{\Ds}{\phi \pip}}
\newcommand{\Dstokstk}{\decay{\Ds}{\Kstarz \Kp}}
\newcommand{\DstToDzPi}{\decay{\Dstarp}{\Dz \pip}}
\newcommand{\DzToMuX}{\decay{\Dz}{\mun X}}
\newcommand{\DmToMuX}{\decay{\Dm}{\mun X}}
\newcommand{\DsToMuX}{\decay{\Dssm}{\mun X}}
\newcommand{\LcToMuX}{\decay{\Lc}{\mup X}}
\newcommand{\DstToDmPiz}{\decay{\Dstarm}{\Dm \piz}}
\newcommand{\DstToDmg}{\decay{\Dstarm}{\Dm \g}}
\newcommand{\DsprimeToDsPiPi}{\decay{D_{s1}(2536)^+}{\Ds\pip\pim}}
\newcommand{\DsoneToDsPiPi}{\decay{D_{s1}(2460)^+}{\Ds\pip\pim}}
\newcommand{\DszToDspiz}{\decay{\Dsz}{\Ds\piz}}
\newcommand{\Jpsimumu}{\decay{\jpsi}{\mup\mun}}

% Excited Ds
\def\Dsz     {{\ensuremath{\D^{*+}_{\squark 0}(2317)}}\xspace}
\def\Dsone     {{\ensuremath{\D_{\squark 1}(2460)^+}}\xspace}
\def\Dsonep     {{\ensuremath{\D_{\squark 1}(2460)^+}}\xspace}
\def\Dsonem     {{\ensuremath{\D_{\squark 1}(2460)^-}}\xspace}
\def\Dsoneexc  {{\ensuremath{\D_{\squark 1}(2536)^-}}\xspace}
\def\Dsstst     {{\ensuremath{\D^{**}_{\squark}}}\xspace}

% lepton decays
\newcommand{\TauToMu}{\decay{\taum}{\mun \neumb \neut}}

% Light decays
\newcommand{\RhoToPiPiz}{\decay{\rhop}{\pip\piz}}

% Form factors decays
\newcommand{\BsToDsst}{\decay{\Bs}{\Dssm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Commenting for early drafts.
\newcommand{\comment}[1]{
\ifreview
	\textit{\color{red}#1}
\else
\fi
}

%% References
\newcommand{\Tabref}[1]{Tab.~\protect\ref{#1}}
\newcommand{\Figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\Secref}[1]{Sec.~\protect\ref{#1}}
\newcommand{\Appref}[1]{App.~\protect\ref{#1}}
\newcommand{\Eqref}[1]{Eq.~\protect\ref{#1}}

%% Luminosity macros
\newcommand{\lumisummary}{\ensuremath{\textit{1024}\invpb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%
\def\tesla   {\textsc{Tesla}\xspace}
\def\loki    {\textsc{LoKi}\xspace}
\def\pidcalib {\textsc{PIDCalib}\xspace}
\def\pythiaeight    {\textsc{Pythia8}\xspace}
\def\geantfour {\textsc{Geant4}\xspace}

% Track quality
\def\IP          {IP\xspace}
\def\ipchisqndof {\ensuremath{\mathrm{IP}\chisq/\mathrm{ndof}}\xspace}
\def\lnchisq     {\ensuremath{\log{\chisq}}\xspace}
\def\ipchisq     {\ensuremath{\chi^2_{\rm IP}}\xspace}
\def\lnipchisq   {\ensuremath{\ln{\chi^2_{\rm IP}}}\xspace}

% PID
\def\probnnk {\mathrm{ProbNN\ensuremath{k}}\xspace}

% Rs
\def\RDp      {{\ensuremath{\mathcal{R}(\Dp)}}\xspace}
\def\RDz      {{\ensuremath{\mathcal{R}(\Dz)}}\xspace}
\def\RD       {{\ensuremath{\mathcal{R}(\D)}}\xspace}
\def\RDst     {{\ensuremath{\mathcal{R}(\Dstar)}}\xspace}
\def\RDs      {{\ensuremath{\mathcal{R}(\Ds)}}\xspace}
\def\RDss     {{\ensuremath{\mathcal{R}(\Dss)}}\xspace}


% LHCb trigger jargon
\def\tis    {TIS\xspace}
\def\tos    {TOS\xspace}
\def\tistos {\tis{}\tos{}\xspace}

% efficiencies

\def\etrigD {\ensuremath{\varepsilon_{\mathrm{trig}}^{\mathrm{data}}}\xspace}
\def\etrigMC{\ensuremath{\varepsilon_{\mathrm{trig}}^{\mathrm{sim}}}\xspace}
\def\etrackD {\ensuremath{\varepsilon_{\mathrm{track}}^{\mathrm{data}}}\xspace}
\def\etrackMC{\ensuremath{\varepsilon_{\mathrm{track}}^{\mathrm{sim}}}\xspace}
\def\corrBs {\ensuremath{c_{\mathrm{kin}}^{\Bs}}\xspace}
\def\corrg  {\ensuremath{c_{\mathrm{kin}}^{\g}}\xspace}
\def\egen   {\ensuremath{\varepsilon_{\mathrm{acc\times rec\times trig\times sel}}}\xspace}
\def\esel   {\ensuremath{\varepsilon_{\mathrm{sel}}^{\Dsm}}\xspace}
\def\ephot  {\ensuremath{\varepsilon_{\mathrm{sel}, \g}}\xspace}
\def\epid   {\ensuremath{\varepsilon_{\mathrm{PID}}}\xspace}


\def\w {\ensuremath{w}\xspace}
\def\wrec {\ensuremath{w_{\rm rec}}\xspace}
\def\wtrue {\ensuremath{w_{\rm true}}\xspace}
\def\wunf {\ensuremath{w_{\rm unf}}\xspace}
\def\mcorr {\ensuremath{m_{\rm corr}}\xspace}


\def\mDss {\ensuremath{m_{\Dssm}}\xspace}
\def\mDsssq {\ensuremath{m_{\Dssm}^2}\xspace}
\def\mDsssqsq {\ensuremath{m_{\Dssm}^4}\xspace}
\def\mBssq {\ensuremath{m_{\Bs}^2}\xspace}
\def\mBssqsq {\ensuremath{m_{\Bs}^4}\xspace}

% angles
\def\thetal {\ensuremath{\theta_{\mu}}\xspace}
\def\thetaV {\ensuremath{\theta_{D_s}}\xspace}


